Autonomous Drone Racing with Deep Reinforcement Learning

In many robotic tasks, such as autonomous drone racing, the goal is to travel through a set of waypoints as fast as possible. A key challenge for this task is planning the time-optimal trajectory, which is typically solved by assuming perfect knowledge of the waypoints to pass in advance. The resulting solution is either highly specialized for a single-track layout, or suboptimal due to simplifying assumptions about the platform dynamics. In this work, a new approach to near-time-optimal trajectory generation for quadrotors is presented. Leveraging deep reinforcement learning and relative gate observations, our approach can compute near-time-optimal trajectories and adapt the trajectory to environment changes. Our method exhibits computational advantages over approaches based on trajectory optimization for non-trivial track configurations. The proposed approach is evaluated on a set of race tracks in simulation and the real world, achieving speeds of up to 60 km/h with a physical quadrotor.

==> figures/figures_final/computation_time.tex <==
% This file was created by tikzplotlib v0.9.8.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.67843137254902,0.847058823529412,0.901960784313726}
\definecolor{color1}{rgb}{ 0.49, 0.8, 0.63}
\definecolor{color3}{rgb}{0.13, 0.6, 0.33}
\definecolor{color4}{rgb}{0.13, 0.38, 0.55}


\begin{axis}[
legend cell align={left},
height=5.5cm,
width=0.93\linewidth,
xmajorgrids,ymajorgrids,
legend style={
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=white!80!black
},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Track Length [m]},
xmin=41.025, xmax=473.435,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Computation Time [hours]},
ymin=-1.00583333333333, ymax=23.3225,
ytick style={color=black},
ytick={0, 5, 10, 15, 20}
]

\addplot [line width=1.5pt, color0, forget plot]
table {%
60.68 -0.018979251239442
61.45 0.00763069780053893
69.31 0.260204041611003
71.01 0.310412633276866
186.25 1.5153812804616
189.09 1.52537573867877
197.96 1.56198143493898
223.31 1.73963979444244
333.63 5.65854002761561
381.83 10.2011196130975
391.72 11.4303434694463
395.31 11.9041744245777
453.78 21.920842761959
};
\addplot [line width=1.5pt, color1, forget plot]
table {%
60.68 1.66185225606159
61.45 1.66820954752649
69.31 1.73071329644337
71.01 1.7436676505663
186.25 2.23804510171522
189.09 2.24268759487573
197.96 2.25551100440344
223.31 2.27976828567311
333.63 2.27973667074067
381.83 2.29608163701793
391.72 2.30550454215923
395.31 2.30958550565848
453.78 2.43863690715846
};

\addplot [draw=color4, fill=color4, mark=*, only marks, scatter/classes={1={mark=square*,color3}}]
table{%
x  y
61.45 0.183333333333333 0
69.31 0.233333333333333 0
60.68 0.1 0
197.96 2.33333333333333 0
189.09 1.15 0
186.25 1.96666666666667 0
395.31 11.7833333333333 0
391.72 11.9666666666667 0
381.83 8.58333333333333 0
453.78 22.2166666666667 0
223.31 0.766666666666667 0
333.63 6.6 0
71.01 0.133333333333333 0
};
\addlegendentry{CPC}

\addplot [draw=color3, fill=color3, mark=*, only marks, scatter/classes={1={mark=square*,color3}}]
table{%
x  y
61.45 1.93333333333333 1
69.31 2.26666666666667 1
60.68 2.28333333333333 1
197.96 2.18333333333333 1
189.09 2.31666666666667 1
186.25 2.25 1
395.31 2.33333333333333 1
391.72 2.41666666666667 1
381.83 1.9 1
453.78 1.86666666666667 1
223.31 2.25 1
333.63 2.3 1
71.01 1.15 1
};
\addlegendentry{Ours}
\end{axis}

\end{tikzpicture}

==> figures/figures_sub/computation_time.tex <==
% This file was created by tikzplotlib v0.9.8.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.67843137254902,0.847058823529412,0.901960784313726}
\definecolor{color1}{rgb}{ 0.49, 0.8, 0.63}
\definecolor{color3}{rgb}{0.13, 0.6, 0.33}
\definecolor{color4}{rgb}{0.13, 0.38, 0.55}


\begin{axis}[
legend cell align={left},
height=5.5cm,
width=0.93\linewidth,
xmajorgrids,ymajorgrids,
legend style={
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=white!80!black
},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Track Length [m]},
xmin=41.025, xmax=473.435,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Computation Time [hours]},
ymin=-1.00583333333333, ymax=23.3225,
ytick style={color=black},
ytick={0, 5, 10, 15, 20}
]

\addplot [line width=1.5pt, color0, forget plot]
table {%
60.68 -0.018979251239442
61.45 0.00763069780053893
69.31 0.260204041611003
71.01 0.310412633276866
186.25 1.5153812804616
189.09 1.52537573867877
197.96 1.56198143493898
223.31 1.73963979444244
333.63 5.65854002761561
381.83 10.2011196130975
391.72 11.4303434694463
395.31 11.9041744245777
453.78 21.920842761959
};
\addplot [line width=1.5pt, color1, forget plot]
table {%
60.68 1.66185225606159
61.45 1.66820954752649
69.31 1.73071329644337
71.01 1.7436676505663
186.25 2.23804510171522
189.09 2.24268759487573
197.96 2.25551100440344
223.31 2.27976828567311
333.63 2.27973667074067
381.83 2.29608163701793
391.72 2.30550454215923
395.31 2.30958550565848
453.78 2.43863690715846
};

\addplot [draw=color4, fill=color4, mark=*, only marks, scatter/classes={1={mark=square*,color3}}]
table{%
x  y
61.45 0.183333333333333 0
69.31 0.233333333333333 0
60.68 0.1 0
197.96 2.33333333333333 0
189.09 1.15 0
186.25 1.96666666666667 0
395.31 11.7833333333333 0
391.72 11.9666666666667 0
381.83 8.58333333333333 0
453.78 22.2166666666667 0
223.31 0.766666666666667 0
333.63 6.6 0
71.01 0.133333333333333 0
};
\addlegendentry{CPC}

\addplot [draw=color3, fill=color3, mark=*, only marks, scatter/classes={1={mark=square*,color3}}]
table{%
x  y
61.45 1.93333333333333 1
69.31 2.26666666666667 1
60.68 2.28333333333333 1
197.96 2.18333333333333 1
189.09 2.31666666666667 1
186.25 2.25 1
395.31 2.33333333333333 1
391.72 2.41666666666667 1
381.83 1.9 1
453.78 1.86666666666667 1
223.31 2.25 1
333.63 2.3 1
71.01 1.15 1
};
\addlegendentry{Ours}
\end{axis}

\end{tikzpicture}

==> tables/gate_displacements.tex <==
\begin{table}[!thp]
\caption{Definition of gate-specific perturbation bounds for Alpha Pilot track. \TODO{this seems redundant if used together with Fig. 6. I like the figure more.}}
\label{tab:gate-displacements}
\begin{center}
\begin{tabular}{| c | c | c | c | c |}
\hline
Gate & $\Delta{x}$ [m]  & $\Delta{y}$ [m]  & $\Delta{z}$ [m] & $\Delta{\alpha} [\circ]$  \\ \hline
1    & [-7.0, 7.0]  & [-7.0, 7.0]   & [-5.0, 5.0] & [-5.0, 5.0]  \\ \hline
2    & [-1.0, 1.0]  & [-1.0, 1.0]   & [-5.0, 5.0] & [-45.0, 45.0]  \\ \hline
3    & [-3.0, 3.0]  & [-3.0, 3.0]   & [-3.0, 3.0] & [-5.0, 5.0]  \\ \hline
4    & [-4.5, 4.5]  & [-4.5, 4.5]   & [-3.0, 3.0] & [-5.0, 5.0]  \\ \hline
5    & [-2.5, 2.5]  & [-2.5, 2.5]   & [-3.0, 3.0] & [-5.0, 5.0]  \\ \hline
6    & [-1.0, 1.0]  & [-1.0, 1.0]   & [-1.0, 1.0] & [-5.0, 5.0]  \\ \hline
7    & [-2.5, 2.5]  & [-2.5, 2.5]   & [-1.0, 1.0] & [-5.0, 5.0]  \\ \hline
8    & [-1.0, 1.0]  & [-1.0, 1.0]   & [-1.0, 1.0] & [-5.0, 5.0]  \\ \hline
9    & [-4.5, 4.5]  & [-4.5, 4.5]   & [-3.0, 3.0] & [-20.0, 20.0]  \\ \hline
10    & [-7.0, 7.0]  & [-7.0, 7.0]   & [-5.0, 5.0] & [-5.0, 5.0]  \\ \hline
11    & [-4.5, 4.5]  & [-4.5, 4.5]   & [-5.0, 5.0] & [-5.0, 5.0]  \\ \hline
\end{tabular}
\end{center}
\end{table}
